RevisEval: Improving LLM-as-a-Judge via Response-Adapted References

With significant efforts in recent studies, LLM-as-a-Judge has become a cost-effective alternative to human evaluation for assessing text generation quality in a wide range of tasks. However, there still remains a reliability gap between LLM-as-a-Judge and human evaluation. One important reason is the lack of guided oracles in the evaluation process. Motivated by the role of reference pervasively used in classic text evaluation, we introduce RevisEval, a novel text generation evaluation paradigm via the response-adapted references. RevisEval is driven by the key observation that an ideal reference should maintain the necessary relevance to the response to be evaluated. Specifically, RevisEval leverages the text revision capabilities of large language models (LLMs) to adaptively revise the response, then treat the revised text as the reference (response-adapted reference) for the subsequent evaluation. Extensive experiments demonstrate that RevisEval outperforms traditional reference-free and reference-based evaluation paradigms that use LLM-as-a-Judge across NLG tasks and open-ended instruction-following tasks. More importantly, our response-adapted references can further boost the classical text metrics, e.g., BLEU and BERTScore, compared to traditional references and even rival the LLM-as-a-Judge. A detailed analysis is also conducted to confirm RevisEval's effectiveness in bias reduction, the impact of inference cost, and reference relevance.

==> section/experiment.tex <==
\section{Experiments}

In this section, we first present the comprehensive experimental settings in Sec.~\ref{sec:setting} and evaluate the \textsc{RevisEval} in LLM-as-a-Judge across various tasks in Sec.~\ref{sec:enhancing}; we then verify the effectiveness of classic text evaluation metrics when using response-adapted references in Sec.~\ref{sec:activating}; building on above findings, we compare two evaluation paradigms, combining LLM-as-a-reviser with multiple metrics and LLM-as-a-Judge, when using weak LLM in Sec.~\ref{sec:potential}; finally, we conduct detailed comparative analysis of \textsc{RevisEval} in Sec.~\ref{sec:comparative_analysis}, such as bias reduction, inference cost impact and reference relevance.


\subsection{Evaluation Settings}
\label{sec:setting}
\paragraph{Evaluation benchmarks.} We evaluate our approach on multiple classic NLG benchmarks by measuring the correlation between the evaluators/metrics and human annotations in a \textbf{scoring rating} task. We follow the experimental setting of~\citet{jiang2024tigerscore} and select four representative NLG tasks: \textbf{Data-to-Text}, \textbf{Machine Translation}, \textbf{Text Summarization}, and \textbf{Story Generation}. Table~\ref{tab:statistic_nlg} shows the details of these benchmarks. Additionally, we test our approach on the more challenging open-ended instruction-following benchmarks (\textbf{MT-Bench}, \textbf{Alpacafarm}, and \textbf{LLMBar}), which primarily rely on \textbf{pairwise comparison} task. Unlike the NLG benchmarks, these preference datasets contain more general instructions covering a broader range of tasks with more diverse responses.



\begin{table*}[!t]
\centering
\small 
\caption{Kendall ($\tau$) and Spearman ($\rho$) correlation results comparing reference-free, reference-based, and \textsc{RevisEval} methods across natural language generation tasks. This table demonstrates that, without human-annotated references, our proposed \textsc{RevisEval} significantly outperforms reference-free and reference-based methods involving both open-source and proprietary LLM-as-a-Judge.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule

\multirow{2}{*}{\textbf{Methods}}& \textbf{\textsc{Summarization}} & \textbf{\textsc{Translation} }& \textbf{\textsc{Data2Text}} & \textbf{\textsc{Story Generation}} & \textbf{Avg.}\\
 & \multicolumn{1}{c}{\bf $\tau$/$\rho$} & \multicolumn{1}{c}{\bf $\tau$/$\rho$} & \multicolumn{1}{c}{\bf $\tau$/$\rho$} & \multicolumn{1}{c}{\bf $\tau$/$\rho$} & \multicolumn{1}{c}{\bf $\tau$/$\rho$}\\
\midrule
\multicolumn{6}{c}{N-gram Metrics} \\
\midrule
\textbf{BLEU} & 10.66/14.42& 14.50/19.73&23.13/33.29&-1.93/-2.70&11.59/16.19\\
\textbf{ROUGE} &10.81/14.85& 13.19/17.83&24.74/35.49&-1.53/2.34&11.80/17.63\\
\textbf{METEOR} &12.37/16.72&16.52/18.80&25.58/36.27&-1.87/-2.65&13.15/17.29\\
\midrule
\multicolumn{6}{c}{Model-based Metrics}\\
\midrule
\textbf{BERTScore} &17.50/23.83&31.57/42.41&30.74/43.75&16.00/23.79&23.95/33.45\\
\textbf{BARTScore} &29.12/35.50&7.01/12.83&22.32/34.33&14.15/33.48&18.15/29.04\\
\textbf{UniEval} &\textbf{35.89}/\textbf{47.52}&16.08/21.90& 28.56/38.38&\textbf{31.22}/\textbf{44.46}&27.94/38.07\\
\textbf{GPTScore} &28.20/37.41& 6.50/8.90&19.81/28.82&16.36/23.91 &17.72/24.76\\
\textbf{InstructScore-7B} &20.86/38.68&40.44/\textbf{50.43}&30.21/38.54&13.50/16.13&26.25/35.94\\
\textbf{TIGERScore-7B} &28.79/35.11&33.65/41.50&32.44/42.39 &29.72/39.26&31.15/39.56\\
\textbf{Llama-3.1 8B-Inst}  &27.49/31.02&19.59/23.54&28.46/36.24&26.13/29.97&25.42/30.19\\
\midrule
\multicolumn{6}{c}{Open-Source LLM-as-a-Judge} \\
\midrule
\textbf{Ref-Free}   & 27.83/31.89 & 30.84/38.66 & 38.75/49.32 & 25.74/31.72 & 30.79/37.90 \\
\textbf{Ref-Based}   & 34.09/39.53 & 35.76/41.12 & \textbf{39.24}/50.87 & 8.79/10.44 & 29.47/35.49 \\
\textbf{\textsc{RevisEval} (Ours)}  & 32.41/37.73 & 33.14/39.66& 39.02/49.92 & 25.95/32.11 & \textbf{32.63/39.86}\\

\midrule
\multicolumn{6}{c}{Proprietary LLM-as-a-Judge} \\
\midrule
\textbf{Ref-Free}   & 31.82/38.98 & 34.62/43.38 & 37.99/49.50 & 23.81/33.29 &32.06/41.29 \\
\textbf{Ref-Based} & 32.56/40.01 &  \textbf{41.47}/45.29 &  37.35/49.02 & 17.58/24.86 & 32.24/39.80\\
\textbf{\textsc{RevisEval} (Ours)}  & 33.63/41.15 & 40.72/45.32 & 37.90/\textbf{50.93} & 25.11/35.26 &\textbf{34.34}/\textbf{43.17}\\
\bottomrule
\end{tabular}
}
\label{tab:main_nlg}
\end{table*}




% \end{itemize}

\paragraph{Base LLMs and metrics.} Our proposed \textsc{RevisEval} aims to improve evaluation performance across both LLM-as-a-Judge and classic metrics, offering enhanced results. For \textbf{proprietary LLMs}, we adopt GPT-4 as the base model and focus on implementing our paradigm during the \textbf{inference} stage. For \textbf{open-source LLMs}, we implement our method via \textbf{finetuning} the Llama 3.1-8B model. Following the~\citet{jiang2024tigerscore}'s setting on open-source models, we distill the evaluation outputs generated by GPT-4 when inputting \textit{task instructions and corresponding evaluated responses}, and tune them in our models. Notably, our training data has no overlap with evaluation benchmarks.
For \textbf{classic metrics}, we cover various metrics, like \textit{n-gram based} BLEU, ROUGE, METEOR and \textit{model based} BERTScore, MOVERScore~\citep{zhao2019moverscore}, BARTScore, which rely heavily on references. We validate our method by assessing the utility of \textbf{reference} texts.



We ensure that our approach maintains versatility and fairness across models, with further details on prompts, inference, finetuning, and baselines in the Appendix~\ref{sec:prompt},~\ref{sec:inference},~\ref{sec:finetuning},~\ref{sec:benchmark},~\ref{sec:baselines_nlg} and~\ref{sec:baselines_llm}.


\subsection{Enhancing LLM-as-a-Judge Performance}
\label{sec:enhancing}
We present the main results of our proposed \textsc{RevisEval} across NLG evaluation tasks and instruction-following preference benchmarks in Table~\ref{tab:main_nlg} and~\ref{tab:main_judge}. We summarize the conclusions below.
\paragraph{\textsc{RevisEval} achieves stronger performance across various NLG tasks.}  
For the powerful proprietary LLMs, \textsc{RevisEval} outperforms reference-free and human-annotated reference-based evaluation across tasks with approximately 0.02 in Kendall correlation on average, as demonstrated in Table~\ref{tab:main_nlg}. Notably, in story generation, high-quality human references hinder evaluation for LLM-as-a-Judge, which decreases by 0.06 compared to the reference-free method in the Kendall correlation. In contrast, \textsc{RevisEval} shows that generated response-adapted reference can still significantly enhance evaluation by about 0.08 in Kendall than human reference-based evaluation. An exception is machine translation, where \textsc{RevisEval} aligns closely with reference-based methods, and we analyze this result exists a consistent rationale about reference relevance in Sec~\ref{sec:comparative_analysis}.


For the open-source LLMs, \textsc{RevisEval} not only outperforms the reference-free method but also beats the reference-based methods by over 0.03 on average in Kendall correlation. Especially in story generation, the reference-based approach is consistent with the above conclusion, trailing by approximately 0.17 in Kendall compared to our \textsc{RevisEval}. Furthermore, the LLM with specialized finetuning also performs better than the LLM with general instruction finetuning (\ie, \textit{Llama 3.1-8B Inst}) on NLG evaluation tasks, leading by about 0.02 in Kendall.



\begin{table*}[!t]
\centering
\small 
\caption{Results of LLM-as-a-Judge on instruction-following preference tasks. Our proposed \textsc{RevisEval} significantly enhances the performance of both open-source and proprietary LLM-as-a-Judge across various general evaluation tasks. Here, D.R. denotes Direct Response to instruction.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Methods}  &\textbf{\# of Training Samples}& \textbf{\textsc{MT-Bench}} & \textbf{\textsc{AlpacaFarm}} & \textbf{\textsc{LLMBar}} & \textbf{Avg.}\\
\midrule
\multicolumn{6}{c}{Open-Source LLM-as-a-Judge} \\
\midrule
\textbf{JudgeLM-7B}~\citep{zhu2023judgelmfinetunedlargelanguage}&100,000&64.1&53.9&36.3&51.4\\
\textbf{PandaLM-7B}~\citep{wang2024pandalm}&300,000&75.0&54.9&31.7&53.9\\
\textbf{Auto-J-13B}~\citep{li2024generative}&4,396&75.2&64.6&36.0&58.6\\
\textbf{Prometheus-7B}~\citep{kim2024prometheus}&100,000&52.8&33.5&30.1&38.8\\
\textbf{Prometheus-2-7B}~\citep{kim2024prometheus2opensource} &300,000&55.0&37.3&26.3&39.5\\
\midrule

\textbf{Llama 3.1-8B-Tuned} &&&&\\
\quad--\textbf{Ref-Free} &9,800&67.4& 61.1&51.1 &59.9 \\
\quad--\textbf{Ref-Based (Llama-D.R.)}    &9,800&74.9&61.5&58.9 &65.1\\%608591  534
\quad--\textbf{Ref-Based (GPT-4-D.R.)} &9,800&78.0&  65.5 & 63.0 & 68.8\\
\quad--\textbf{\textsc{RevisEval} (Llama-as-a-Reviser)}&9,800&75.2& 64.7 & 57.8 & 65.9\\
\quad--\textbf{\textsc{RevisEval} (GPT-4-as-a-Reviser)} &9,800&79.3& 67.1 & 64.9 & 70.4\\

\midrule
\multicolumn{6}{c}{Proprietary LLM-as-a-Judge (GPT-4)} \\
\midrule
\textbf{Ref-Free}  &-&81.2&70.9&72.6 &74.9\\
\textbf{Ref-Based (GPT-4-D.R.)}   &-&81.5&67.7&\textbf{79.9}&76.4\\
\textbf{\textsc{RevisEval} (GPT-4-as-a-Reviser)} &-&\textbf{83.0}&\textbf{72.9}& 79.0 &\textbf{78.1}\\
\bottomrule
\end{tabular}
}
\label{tab:main_judge}
\end{table*}



\paragraph{\textsc{RevisEval} excels on open-ended instruction-following preference benchmarks.} As shown in Table~\ref{tab:main_judge},
whether implemented on open-source or proprietary models, \textsc{RevisEval} consistently surpasses all baselines by at least 6.3\% on average. The details of these baselines are listed in Appendix~\ref{sec:baselines_llm}, and they are tuned with tens of thousands of data for the LLM-as-a-Judge. On the same base LLM, \textsc{RevisEval} exceeds reference-free evaluation by 3\%-6\%. We compare \textsc{RevisEval} to reference-based evaluations followed by \citet{zheng2023judging}'s setup, whose reference is the LLM's direct response to the instruction. Our approach performs better than reference-based evaluation on average when both references are generated by the same base LLMs. Furthermore, using GPT-4 as the reviser boosts Llama 3.1-8B-as-a-Judge by over 4.5\% compared to Llama-as-a-Reviser, highlighting the importance of reference quality.

LLM-as-a-Judge can be biased toward longer, verbose answers~\citep{saito2023verbosity,dubois2024lengthcontrolledalpacaevalsimpleway} or answers that match a similar format~\citep{huang2024limitations}. LLMBar~\citep{zeng2024evaluating} is a challenging benchmark to meta-evaluate such superficial quality biases.
As demonstrated in Table~\ref{tab:main_judge}, these baselines, even after tuning $>100K$ samples, struggle to exceed 50\% accuracy, exposing bias challenge significantly.
%This improvement is even more pronounced with weaker open-source LLMs as evaluators, where baselines, even after extensive tuning, struggled to exceed 50\% accuracy. 
By using response-adapted references from \textsc{RevisEval}, the weak open-source LLM-as-a-Judge's performance improves substantially by about 6\%, showing \textbf{\textsc{RevisEval} can address superficial quality bias}. 
On proprietary LLM, \textsc{RevisEval} achieves a 3.2\% improvement in accuracy compared to reference-free evaluation. Our proposed response-adapted references perform slightly worse than direct responses from the same proprietary model. This is likely because LLMBar emphasizes ``instruction-following precision,'' where a single ground-truth response exists for the instruction.


In summary, \textsc{RevisEval} consistently outperforms traditional reference-free and reference-based methods, and our revision significantly provides guidance for LLM evaluation by significantly utilizing the generative advantages of LLM. %eliminating the reliance on human-generated references. 



\subsection{Activating classic metrics Performance}
\label{sec:activating}
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.95\textwidth]{figure/metrics.pdf}
\end{center}
\caption{Comparative analysis of reference-based metrics performance using references generated by \textsc{Human/GPT-4} and \textsc{RevisEval} on NLG and instruction following benchmarks. \textsc{RevisEval} can greatly enhance traditional reference-based metrics, even n-gram metrics, reaching performance levels comparable to GPT-4-as-a-Judge in reference-free evaluations.}
\label{fig:metrics}
\end{figure}

%Comparative analysis of reference-based metrics performance using references generated by \textsc{Human/GPT-4} and \textsc{RevisEval} on NLG and instruction following benchmarks. \textsc{RevisEval} can greatly enhance traditional reference-based metrics, even n-gram metrics, reaching performance levels comparable to GPT-4-as-a-Judge in reference-free evaluations. 

Since response-adapted references have enhanced LLM-as-a-Judge in Sec.~\ref{sec:enhancing}, this motivates us to ask \textit{could these references directly improve the performance of classic metrics, even n-gram metrics}?

As the classic text metrics are not compatible with the pairwise comparison, we extend them as follows:
\begin{center}
    $s = \mathbb{I}(\mathcal{F}_M(y_1,r) > \mathcal{F}_M(y_2,r)),$
\end{center}
where \(\mathbb{I}(\cdot)\) is the indicator function, determining which $y_1$ or $y_2$ is preferred based on the metric scores.
We use human references in NLG tasks and GPT-4 direct responses in instruction-following benchmarks as the baseline references $\hat{r}$, comparing them with references $r^\star$ generated by \textsc{RevisEval}. As shown in Figure~\ref{fig:metrics}, \textsc{RevisEval} enables each classic metric to significantly surpass its performance based on baseline references across all tasks. This increase is especially evident in more complex open-ended tasks like story generation and AlpacaFarm. Additionally, we find that using $r^\star$ generated by GPT-4 as-a-Reviser combined with classic metrics can yield comparable evaluation performance to GPT-4's reference-free evaluation. Notably, in AlpacaFarm, when using the response-adapted references, MOVERScore achieves 1.2\% improvement compared to the reference-free GPT-4-as-a-Judge.

\subsection{Potential Evaluation Paradigm for Weak Large Language Models}
\label{sec:potential}
\begin{table*}[!t]
\centering
\small 
\caption{Comparative analysis of weak \textbf{LLM-as-a-Judge} and weak \textbf{LLM-as-a-Reviser+classic metrics} on instruction-following tasks. Under the same finetuning training resources, a weak LLM-as-a-Reviser combined with classic metrics can produce better results.}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Metrics}  & \textbf{\textsc{MT-Bench}} & \textbf{\textsc{AlpacaFarm}}& \textbf{\textsc{LLMBar}} & \textbf{Avg.}\\
\midrule
\textbf{LLM-as-a-Reviser} &&&&\\
\quad\textbf{BLEU} &64.5&63.9&51.6& 60.0\\
\quad\textbf{ROUGE} &62.0&63.5&51.6&59.0\\
\quad\textbf{METEOR} &66.4&67.7&46.3&60.1\\
\quad\textbf{BERTScore} &62.3&62.3&\textbf{54.4}&59.7\\
\quad\textbf{MOVERScore}&61.5&68.3&51.6&60.5\\
\quad\textbf{BARTScore} &66.9&61.9&51.3&60.0\\
\quad\textbf{\textsc{Majority Voting}} &63.4&\textbf{68.5}&52.5&\textbf{61.4}\\
\midrule
\textbf{LLM-as-a-Judge} &\textbf{67.4}&61.1& 51.1 &59.9\\  
\bottomrule
\end{tabular}
}
\label{tab:potential}
\end{table*}


We observe that 1) in the Sec.~\ref{sec:enhancing}, all weak LLMs still exhibit a significant gap compared to GPT-4-as-a-Judge, even after extensive training with high-quality, evaluation-specific data, and 2) in the Sec.~\ref{sec:activating}, classic metrics combined with response-adapted references generated by GPT-4 can achieve performance close to the reference-free GPT-4-as-a-Judge. Thus, \textit{should we consider a potential evaluation paradigm of ``weak LLM-as-a-Reviser + metrics'' instead of ``weak LLMs-as-a-Judge''?}

To explore this, we compare ``Llama-as-a-Judge'' with ``Llama-as-a-Reviser + metrics,'' as shown in Table~\ref{tab:potential}. When using references generated by ``Llama-as-a-Reviser'', we find that BLEU, METEOR, MOVERScore, and BARTScore can surpass ``Llama-as-a-Judge'' on average across 3 tasks. Furthermore, we apply a \textit{majority voting} across multiple metrics, outperforming ``Llama-as-a-Judge'' over 1.5\% on average. This suggests that instead of continuously training weak LLMs to improve their evaluative \textbf{discrimination} capabilities, leveraging their \textbf{generation} abilities for revision may be more effective. Without extra inference costs, this approach can lead to better evaluation outcomes.


\begin{table*}[hbt!]
\centering
\small 
\caption{Positional bias analysis in pair comparison evaluations when applying different evaluation paradigms. This table presents the ratio of changed evaluation results after swapping the response position. A lower proportion indicates less positional bias.\textsc{RevisEval} stands out as the best, exhibiting the lowest bias among all paradigms.}
\resizebox{0.97\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Paradigms}}&\multicolumn{2}{c}{\textbf{\textsc{MT-Bench}}}&\multicolumn{2}{c}{\textbf{\textsc{Alpacafarm}}}&\multicolumn{2}{c}{\textbf{\textsc{LLMBar}}}\\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
&\textsc{Llama 3.1-8B}&\textsc{GPT-4}&\textsc{Llama 3.1-8B}&\textsc{GPT-4}&\textsc{Llama 3.1-8B}&\textsc{GPT-4}\\
\midrule
\textbf{Ref-Free} &49.1 &10.3&61.1&20.0&44.6&17.9\\
\textbf{Ref-Based} &22.8&6.5 &34.1&22.2&32.5&11.2\\
\textbf{\textsc{RevisEval}} &\textbf{20.5} &\textbf{5.9}&\textbf{30.1}&\textbf{19.9}&\textbf{30.3}&\textbf{7.9}\\
\bottomrule
\end{tabular}
}
\label{tab:positional_bias}

\end{table*}

\subsection{Comparative Analysis to Other Evaluation Paradigms}
\label{sec:comparative_analysis}


\paragraph{Positional bias analysis.} Positional bias~\citep{wang2024large,zheng2023judging,wu2023style,chen2024humans} occurs when human or LLM evaluators tend to favor one side in a pairwise comparison, regardless of answer quality. We investigate this bias by swapping answer positions and taking the LLM to re-evaluate, as shown in Table~\ref{tab:positional_bias}. The results indicate that reference-based evaluation decisions have less variation than reference-free ones. \textsc{RevisEval} is generally 2\%-4\% lower on the reference-based evaluation, showing better consistency. This result is probably because \textsc{RevisEval} provides references more closely aligned with the answers, further minimizing bias. 




\begin{table*}[!t]
\centering
\small 
\caption{Ablation study on the impact of inference cost. Increasing evaluation cycles to match or exceed \textsc{RevisEval}'s inference cost in reference-free did not improve accuracy. This shows that \textsc{RevisEval}'s superior performance is not from twice inference.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Inference Cost}}  &\multicolumn{2}{c}{\textbf{\textsc{MT-Bench}}} &\multicolumn{2}{c}{\textbf{\textsc{AlpacaFarm}}}  &\multicolumn{2}{c}{\textbf{\textsc{LLMBar}}}\\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
&\textsc{Llama 3.1-8B}&\textsc{GPT-4}&\textsc{Llama 3.1-8B}&\textsc{GPT-4}&\textsc{Llama 3.1-8B}&\textsc{GPT-4}\\
\midrule
\textbf{1-Cycle Ref-Free}  &67.4 &81.2 &61.1 &70.9&51.1 &72.6\\
%\textbf{\textsc{2-Cycle Vanilla}}  &63.6 &80.5 &57.3 &66.5&48.7 &73.0\\
\textbf{3-Cycle Ref-Free}  &64.1 &81.2 &54.9 &71.9 &53.2 &74.9\\
\midrule

\textbf{\textsc{RevisEval} (2-Cycle)} &\textbf{71.3} &\textbf{83.0} &\textbf{64.7}&\textbf{72.9}  &\textbf{54.9}&\textbf{79.0}\\
\bottomrule
\end{tabular}
}
\label{tab:inference_cost}
\end{table*}


\paragraph{The impact analysis of inference cost.}  
Compared to the reference-free approach, \textsc{RevisEval}  requires two cycles of inference (\ie, revision and evaluation). To show the impact of extra inference cost, we further 
conduct three cycles of reference-free evaluations using extra different temperatures ($0.3$ and $0.7$), followed by majority voting (see Table~\ref{tab:inference_cost}). For GPT-4, additional evaluation cycles slightly improve accuracy but still lag behind ours by 1\%-4\%. For weak LLMs, more cycles led to worse performance. The above results indicate that our approach provides more valuable guidance.




\begin{table*}[!t]
    \centering
    \caption{Comparative analysis of how reference-based evaluation effectiveness varies with changes in the similarity between the response and reference texts across different constructing reference strategies. Here, Effectiveness, $\mathcal{P}_{\text{ref}}/\mathcal{P}_{\text{free}}$, refers to the performance ratio between reference-based and reference-free evaluation, where $\mathcal{P}$ denotes the evaluation performance, \eg, $\text{Acc}$ and $\text{Corr}$; similarity is still measured by BERTScore.}
        \label{tab:similarity}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccccccc}
            \toprule
&\textbf{Reference Source}& \textbf{\textsc{WMT-22(en-zh)}} & \textbf{\textsc{WebNLG}} & \textbf{\textsc{MT-Bench}}  & \textbf{\textsc{Summeval}}  & \textbf{\textsc{AlpacaFarm}} &  \textbf{\textsc{ROC}} \\
\midrule
 \multirow{2}{*}{\textbf{Similarity}} &Human/GPT-4 & \textbf{65.12}  & 59.09  & 25.00 & 23.51 & 13.04 & 12.86   \\
&RevisEval & 63.03 (\red{-3.3\%}) & \textbf{76.41} (\green{+29.3\%}) & \textbf{30.29} (\green{+21.2\%}) & \textbf{35.63} (\green{+51.6\%})  & \textbf{35.72} (\green{+173.9\%}) & \textbf{27.57} (\green{+114.4\%}) \\
            \midrule
            \multirow{2}{*}{\textbf{Effectiveness}} &Human/GPT-4 & \textbf{1.20} & 0.98& 1.00& 1.02  & 0.95& 0.74  \\
            &RevisEval & 1.18 (\red{-0.02}) & \textbf{1.00} (\green{+0.02}) & \textbf{1.02} (\green{+0.02})& \textbf{1.06} (\green{+0.04}) &\textbf{ 1.03} (\green{+0.08})& \textbf{1.05} (\green{+0.31})\\
                  \bottomrule
        \end{tabular}
  
    }
    \end{table*}
\paragraph{Evaluation performance improves with increased relevance between reference and responses.} 
It's been observed that the less relevant a reference is to the response, the less effective it is for evaluation in previous work and Figure~\ref{fig:pilot}. We further verify whether this trend holds true with our method. 
We define effectiveness to describe whether reference-based evaluation is more effective than reference-free evaluation.
As shown in Table~\ref{tab:similarity}, the increasing similarity between reference and evaluated responses generally leads to better evaluation effectiveness. This explains why our method doesn't perform as well in translation, where human references are already highly similar to the response. For other tasks, human or GPT-4 direct-response references have lower similarity than references of \textsc{RevisEval}, leading to a lower effectiveness. Additionally, for different tasks, the similarity between the human/GPT-4 reference and the evaluated response varies, reflecting the open-ended generative degree of this task. A lower similarity indicates a greater diversity of potential valid responses. In this context, as the task becomes more open-ended, the effectiveness of \textsc{RevisEval} shows a greater improvement than the human/GPT-4 reference.










